Heterogeneous interventional indirect effects with multiple mediators: non-parametric and semi-parametric approaches

We propose semi- and non-parametric methods to estimate conditional interventional effects in the setting of two discrete mediators whose causal ordering is unknown. Average interventional indirect effects have been shown to decompose an average treatment effect into a direct effect and interventional indirect effects that quantify effects of hypothetical interventions on mediator distributions. Yet these effects may be heterogeneous across the covariate distribution. We consider the problem of estimating these effects at particular points. We propose an influence-function based estimator of the projection of the conditional effects onto a working model, and show under some conditions that we can achieve root-n consistent and asymptotically normal estimates. Second, we propose a fully non-parametric approach to estimation and show the conditions where this approach can achieve oracle rates of convergence. Finally, we propose a sensitivity analysis for the conditional effects in the presence of mediator-outcome confounding. We propose estimating bounds on the conditional effects using these same methods, and show that these results easily extend to allow for influence-function based estimates of the bounds on the average effects. We conclude examining heterogeneous effects with respect to the effect of COVID-19 vaccinations on depression during February 2021.

==> tables/drl-table-gt.tex <==
\captionsetup[table]{labelformat=empty,skip=1pt}
\begin{longtable}{rlrrrrrlrrrrl}
\caption*{
{\large Non-parametric estimators: simulation performance}
} \\ 
\toprule
 &  &  & \multicolumn{5}{c}{CIIE-M1} & \multicolumn{5}{c}{CATE} \\ 
\cmidrule(lr){4-8} \cmidrule(lr){9-13}
Point & Strategy & N & Truth & Bias & Std & RMSE & Coverage & Truth & Bias & Std & RMSE & Coverage \\ 
\midrule
0 & DRLearner & 1000 & $0.071$ & $0.002$ & $0.081$ & $0.081$ & 94.3 & $0.092$ & $-0.004$ & $0.074$ & $0.074$ & 93.7 \\ 
0 & DRLearner & 2000 & $0.071$ & $0.002$ & $0.055$ & $0.055$ & 95.5 & $0.092$ & $-0.009$ & $0.054$ & $0.054$ & 93.2 \\ 
0 & Plug-in & 1000 & $0.071$ & $-0.004$ & $0.030$ & $0.030$ & - & $0.092$ & $-0.010$ & $0.059$ & $0.060$ & - \\ 
0 & Plug-in & 2000 & $0.071$ & $-0.003$ & $0.020$ & $0.020$ & - & $0.092$ & $-0.012$ & $0.042$ & $0.043$ & - \\ 
2 & DRLearner & 1000 & $0.113$ & $-0.002$ & $0.107$ & $0.107$ & 92.6 & $0.131$ & $0.008$ & $0.081$ & $0.081$ & 91.9 \\ 
2 & DRLearner & 2000 & $0.113$ & $-0.004$ & $0.062$ & $0.062$ & 93.6 & $0.131$ & $0.011$ & $0.057$ & $0.058$ & 93 \\ 
2 & Plug-in & 1000 & $0.113$ & $-0.040$ & $0.027$ & $0.048$ & - & $0.131$ & $0.014$ & $0.060$ & $0.062$ & - \\ 
2 & Plug-in & 2000 & $0.113$ & $-0.040$ & $0.020$ & $0.044$ & - & $0.131$ & $0.011$ & $0.043$ & $0.045$ & - \\ 
\bottomrule
\end{longtable}



==> tables/drl-table.tex <==
% latex table generated in R 4.2.0 by xtable 1.8-4 package
% Wed Jul 20 12:54:05 2022
\begin{table}[ht]
\centering
\caption{Non-parametric estimators: simulation performance} 
\label{tab:sim2}
\begin{tabular}{rlrrrrrl}
  \hline
Point & Strategy & N & Truth & Bias & Std & RMSE & Coverage \\ 
  \hline
  0 & DRLearner & 1000 & 0.07 & 0.00 & 0.08 & 0.08 & 94.3 \\ 
    0 & DRLearner & 2000 & 0.07 & 0.00 & 0.06 & 0.06 & 95.5 \\ 
    0 & Plug-in & 1000 & 0.07 & -0.00 & 0.03 & 0.03 & - \\ 
    0 & Plug-in & 2000 & 0.07 & -0.00 & 0.02 & 0.02 & - \\ 
    2 & DRLearner & 1000 & 0.11 & -0.00 & 0.11 & 0.11 & 92.6 \\ 
    2 & DRLearner & 2000 & 0.11 & -0.00 & 0.06 & 0.06 & 93.6 \\ 
    2 & Plug-in & 1000 & 0.11 & -0.04 & 0.03 & 0.05 & - \\ 
    2 & Plug-in & 2000 & 0.11 & -0.04 & 0.02 & 0.04 & - \\ 
   \hline
\end{tabular}
\end{table}


==> text/identification.tex <==
%\begin{proof}[Identification]\label{proof0}

%Assume equations (\ref{eqn:unconf1})-(\ref{eqn:unconf3}). Let $G_{a}(M_1 \mid X) \sim p(M_1^a \mid X)$, $G_{a'}(M_1 \mid X) \sim p(M_1^{a'} \mid X)$, and $G_{a'}(M_2 \mid X) \sim p(M_2^{a'} \mid X)$. Then $G_{a\star}(M_1 \mid X) \perp Y^{am_1m_2} \mid X$ and $G_{a^\star}(M_2 \mid X) \perp Y^{am_1m_2} \mid X$ for $a^\star \in \{a, a'\}$. We then see:

%\begin{align}
%    \label{eqn:identn1}\psi_{M_1} &= \int_X \mathbb{E}[Y^{aG_a(M_1 \mid X)G_{a'}(M_2 \mid X)} \mid X] - \mathbb{E}[Y^{aG_{a'}(M_1 \mid X)G_{a'}(M_2 \mid X)} \mid X]dP(X) \\
%    \label{eqn:ident0} &= \int_X[\sum_{m_1, m_2}\mathbb{E}[Y^{am_1m_2} \mid X, G_a(M_1 \mid X) = m_1, G_a(M_2 \mid X) = m_2] \\ 
%    \nonumber&\times p(G_a(M_1 \mid x) = m_1) p(G_{a'}(M_2 \mid X) = m_2) \\
%    \nonumber &- \mathbb{E}[Y^{am_1m_2} \mid X, G_{a'}(M_1 \mid X) = m_1, G_a(M_2 \mid X) = m_2)] \\
%    \nonumber &\times p(G_{a'}(M_1 \mid X) = m_1)p(G_{a'}(M_2 \mid X) = m_2))]dP(X) \\
%    \label{eqn:ident0a} &= \int_X[\sum_{m_1, m_2}\mathbb{E}[Y^{am_1m_2} \mid X][p(G_a(M_1 \mid x) = m_1)p(G_{a'}(M_2 \mid X) = m_2) \\
%    \nonumber &- p(G_{a'}(M_1 \mid X) = m_1)p(G_{a'}(M_2 \mid X) = m_2)]dP(X) \\
%    \label{eqn:ident1}&= \int_X\left(\sum_{m_1, m_2}\mathbb{E}[Y^{am_1m_2} \mid X, a, m_1, m_2]\{p(M_1^a = m_1 \mid X) - p(M_1^{a'} = m_1 \mid X)\}p(M_2^{a'} = m_2 \mid X)dP(X)\right) \\
%    \label{eqn:ident3}&= \mathbb{E}\left(\sum_{m_1, m_2}\mathbb{E}[Y \mid X, a, m_1, m_2]\{p(m_1 \mid X, A = a) - p(m_1 \mid X, A = a')\}p(m_2 \mid X, A = a')\right) \\
%    \label{eqn:ident6}&= \mathbb{E}\left(\sum_{m_1, m_2}\mu_a(X, m_1, m_2)\{p(m_1 \mid X, a) - p(m_1 \mid X, a')\}p(m_2 %\mid X, a')\right)
%\end{align}
%
%where \eqref{eqn:identn1} follows by definition and by iterating expectation on $X$, \eqref{eqn:ident0} by iterating expectations, \eqref{eqn:ident0a} by randomization of $G_a(M_1 \mid X)$, $G_{a'}(M_1 \mid X)$, and $G_{a'}(M_2 \mid X)$, \eqref{eqn:ident1} by definition of $G_a$ and by $Y-A$ and $Y-M$ randomization, \eqref{eqn:ident3} by $M-A$ randomization, and \eqref{eqn:ident6} by consistency.
%\end{proof}


==> text/second-order-terms.tex <==
In this section we re-derive the second-order reminder of the influence function based estimator for $\psi_{M_1}$ to show that this can be expressed as a product of errors in the nuisance estimation.

\section{Background}

Consider the functional:

\begin{align}
    \psi_{M_1} &= \sum_{x, m_1, m_2}\mathbb{E}[Y \mid m_1, m_2, a, x][p(m_1 \mid a, x) - p(m_1 \mid a', x)]p(m_2 \mid a', x)p(x) \\
    &= \psi_{M_1, a} - \psi_{M_1, a'}
\end{align}

Let $O = (Y, A, X, M_1, M_2)$. We define the following functions of the data:

\begin{align*}
&\mu_{a, M_1\times M_2'}(X) = \sum_{m_1, m_2}\mu_a(m_1, m_2, X)p(m_1 \mid a, X)p(m_2 \mid a', X)  \\
&\mu_{a, M_1^'}(M_2, X) = \sum_{m_1}\mu_a(m_1, M_2, X)p(m_1 \mid a', X)
\end{align*}
%
and so forth. The influence curve of $\psi_{a, M_1}$ takes the following form:

\begin{align}\label{eqn:eifm1}
    \varphi_a(O) &= \frac{\mathds{1}(A = a)}{\pi_a(X)}\frac{p(M_1 \mid a, X)\}p(M_2 \mid a', X)}{p(M_1, M_2, \mid a, X)}(Y - \mu_a(M_1, M_2, X)) \\
    \nonumber &+ \frac{\mathds{1}(A = a)}{\pi_a(X)}\{\mu_{a, M_2^'}(M_1, X) - \mu_{a, M_1\times M_2^'}(X)\} \\ 
    \nonumber &+ \frac{\mathds{1}(A = a')}{\pi_{a'}(X)}\left(\mu_{a, M_1}(M_2, X) - \mu_{a, M_1\times M_2'}(X)\right) \\
    \nonumber &+ \mu_{a, M_1\times M_2^'}(X)
\end{align}

Similarly, the influence curve of $\psi_{M_1, a'}$ takes the following form.

\begin{align}\label{eqn:eifm1}
    \varphi_{a'}(O) &= \frac{\mathds{1}(A = a)}{\pi_a(X)}\frac{p(M_1 \mid a', X)p(M_2 \mid a', X)}{p(M_1, M_2, \mid a, X)}(Y - \mu_a(M_1, M_2, X)) \\
    \nonumber &+ \frac{\mathds{1}(A = a')}{\pi_{a'}(X)}\left(\mu_{a, M_2^'}(M_1, X) - \mu_{a, M_1^'\times M_2^'}(X)\right) \\
    \nonumber &+ \frac{\mathds{1}(A = a')}{\pi_{a'}(X)}\left(\mu_{a, M_1^'}(M_2, X) - \mu_{a, M_1^'\times M_2^'}(X)) \right) \\
    \nonumber &+ \mu_{a, M_1^'\times M_2^'}(X)
\end{align}
%
The influence curve of $\psi_{M_1}$ is then given by:

\begin{align}
    \varphi(O) = \varphi_{a}(O) - \varphi_{a'}(O)
\end{align}

We want to consider the bias of $P[\hat{\varphi}(Z) - \psi_{M_1}]$ and show that this is second-order in the estimation error. Benkenser and Ran (2021) give the following decomposition:

\begin{align}
    \label{eqn:m1decomp.1}&\int \frac{\pi_a(X)}{\hat{\pi}_a(X)}\sum_{m_1, m_2} \left\{\frac{(\hat{p}(m_1 \mid a, X) - \hat{p}(m_1 \mid a', X))(\hat{p}(m_2 \mid a', X))}{p(m_1, m_2 \mid a, X) \hat{p}(m_1, m_2 \mid a, X)}\right\} \\ \nonumber &\times [\hat{\mu}_a(X, m_1, m_2) - \mu_a(X, m_1, m_2)][\hat{p}(m_1, m_2 \mid a, X) - p(m_1, m_2 \mid a, X)]dP(X) \\
    \label{eqn:m1decomp.2}&- \int \left(\frac{\hat{\pi}_a(X) - \pi_a(X)}{\hat{\pi}_a(X)}\right)\sum_{m_1, m_2} (\hat{\mu}_a(X, m_1, m_2) - \mu_a(X, m_1, m_2))\hat{p}(m_1 \mid X, a') \hat{p}(m_2 \mid X, a')dP(X) \\
    \label{eqn:m1decomp.3}&- \int \left(\frac{\hat{\pi}_{a'}(X) - \pi_{a'}(X)}{\hat{\pi}_{a'}(X)}\right)\sum_{m_1, m_2} \mu_a(X, m_1, m_2)[\hat{p}(m_1 \mid, a', X)\hat{p}(m_2 \mid a', X) - p(m_1 \mid a', X)p(m_2 \mid a', X)]dP(X) \\
    \label{eqn:m1decomp.4}&+ \int \left(\frac{\hat{\pi}_{a'}(X) - \pi_{a'}(X)}{\hat{\pi}_{a'}(X)}\right)\sum_{m_1, m_2}\hat{\mu}_a(X, m_1, m_2)\hat{p}(m_1 \mid a, X)[\hat{p}(m_2 \mid a', X) - p(m_2 \mid a', X)]dP(X) \\
    \label{eqn:m1decomp.5}&+ \int \left(\frac{\hat{\pi}_a(X) - \pi_a(X)}{\hat{\pi}_a(X)}\right)\sum_{m_1, m_2} [\hat{\mu}_a(X, m_1, m_2) - \mu_a(X, m_1, m_2)]\hat{p}(m_1 \mid a, X)\hat{p}(m_2 \mid a', X)dP(X) \\
    \label{eqn:m1decomp.6}&+ \int \left(\frac{\hat{\pi}_a(X) - \pi_a(X)}{\hat{\pi}_a(X)}\right)\sum_{m_1, m_2} \hat{\mu}_a(X, m_1, m_2)\hat{p}(m_2 \mid a', X)[\hat{p}(m_1 \mid a, X) - p(m_1 \mid a, X)]dP(X) \\
    \label{eqn:m1decomp.7}&- \int \sum_{m_1, m_2}[\hat{\mu}_a(X, m_1, m_2) - \mu_a(X, m_1, m_2)][\hat{p}(m_1 \mid a, X)\hat{p}(m_2 \mid a', X) - p(m_1 \mid a, X)p(m_2 \mid a', X)]dP(X) \\
    \label{eqn:m1decomp.8}&- \int \sum_{m_1}\sum_{m_2}\hat{\mu}_a(X, m_1, m_2) [\hat{p}(m_2 \mid a', X) - p(m_2 \mid a', X)][\hat{p}(m_1 \mid a, X) - p(m_1 \mid a, X)]dP(X)
\end{align}

I am  suspicious of this result because there it lacks a symmetry that I would expect: specifically, because $\varphi(O) = \varphi_a(O) - \varphi_{a'}(O)$, intuitively we should expect that any terms that exist for $\varphi_{a'}(O)$ should have an analogous term for $\varphi_{a}(O)$. We see that this is the case in \eqref{eqn:m1decomp.1} where this term clearly has components from both of these functionals. On the other hand, \eqref{eqn:m1decomp.8}, which would appear to come from $\varphi_{a}$, does not appear to have an analogous term from $\varphi_{a'}$. I'm also confused why $p(m_1, m_2 \mid a, x)$ appears in the denominator of \eqref{eqn:m1decomp.1}, which I am unable to replicate below.

\section{Decomposition}

Benkeser and Ran (2021) do not provide the algebra associated with their derivation. Therefore, we have to start from scratch. We begin with considering $P[\hat{\psi}_{M_1, a} - \psi_{M_1, a}]$, where $\hat{\psi}_{M_1, a} = P_n[\hat{\varphi}_a(O)]$:

\begin{align}\label{eqn:eifm1a}
    \varphi_a(O) &= \frac{\mathds{1}(A = a)}{\pi_a(X)}\frac{p(M_1 \mid a, X)p(M_2 \mid a', X)}{p(M_1, M_2, \mid a, X)}(Y - \mu_a(M_1, M_2, X)) \\
    \nonumber &+ \frac{\mathds{1}(A = a)}{\pi_a(X)}\{\mu_{a, M_2^'}(M_1, X) - \mu_{a, M_1\times M_2^'}(X)\} \\ 
    \nonumber &+ \frac{\mathds{1}(A = a')}{\pi_{a'}(X)}\left(\mu_{a, M_1}(M_2, X) - \mu_{a, M_1\times M_2'}(X)\right) \\
    \nonumber &+ \mu_{a, M_1\times M_2^'}(X)
\end{align}

\begin{align}
    \nonumber&P[\hat{\varphi}_a(O) - \psi_{M_1, a}] \\
    \nonumber&= \int \frac{\mathds{1}(A = a)}{\hat{\pi}_a(X)}\frac{\{Y - \hat{\mu}_a(M_1, M_2, X)\}\hat{p}(M_1 \mid a, X)\hat{p}(M_2 \mid a, X)}{\hat{p}(M_1, M_2 \mid a, X)}dP(O) \\
    \nonumber&+ \int \frac{\mathds{1}(A = a)}{\hat{\pi}_a(X)}\{\sum_{m_2}\hat{\mu}_a(m_2, M_1, X)\hat{p}(m_2 \mid a', x) - \hat{\mu}_{a, M_1\times M_2^'}(X)\}dP(O) \\
    \nonumber&+ \int \frac{\mathds{1}(A = a')}{\hat{\pi}_{a'}(X)}\left(\hat{\mu}_{a, M_1}(M_2, X) - \hat{\mu}_{a, M_1\times M_2'}(X)\right)dP(O) \\
    \nonumber&+ \int \{\hat{\mu}_{a, M_1\times M_2^'}(X) - \mu_{a, M_1\times M_2^'}(X)\}dP(X) \\
    \label{eqn:d1}&= \int \frac{\pi_a(X)}{\hat{\pi}_a(X)}\sum_{m_1, m_2}\frac{\{\mu_a(m_1, m_2, X) - \hat{\mu}_a(m_1, m_2, X)\}p(m_1, m_2 \mid a, X)\hat{p}(m_1 \mid a, X)\hat{p}(m_2 \mid a, X)}{\hat{p}(m_1, m_2 \mid a, X)}dP(X) \\
    \label{eqn:d2}&+ \int \frac{\pi_a(X)}{\hat{\pi}_a(X)}\left(\sum_{m_1, m_2}\hat{\mu}_a(m_2, m_1, X)\hat{p}(m_2 \mid a', X)(p(m_1 \mid a, X) - \hat{p}(m_1 \mid a, X))\right)dP(X) \\
    \label{eqn:d3}&+ \int \frac{\pi_{a'}(X)}{\hat{\pi}_{a'}(X)}\left(\sum_{m_1, m_2}\hat{\mu}_a(m_1, m_2, X)\hat{p}(m_1 \mid a, x)(p(m_2 \mid a', x) - \hat{p}(m_2 \mid a', X)) \right)dP(X) \\
    \label{eqn:d4}&+ \int \left(\color{red}\hat{\mu}_{a, M_1\times M_2^'}(X)\color{black} - \mu_{a, M_1\times M_2^'}(X)\right)dP(X) 
\end{align}

To ease notation, let $p_1 = p(m_1 \mid a, x)$, $p_2 = p(m_2 \mid a', x)$, $\mu_a = \mu_a(m_1, m_2, x)$, and $\pi_a = \pi_a(X)$. We also remove the integrals over the distribution of $X$ and leave this as implied. First, consider \eqref{eqn:d1}:

\begin{align*}
    &= \underbrace{\frac{\pi_a}{\hat{\pi}_a}\sum_{m_1, m_2}\frac{(\mu_a - \hat{\mu}_a)(p_{12} - \hat{p}_{12})\hat{p}_1\hat{p}_2}{\hat{p}_{12}}}_{(i)} + \frac{\pi_a}{\hat{\pi}_a}\sum_{m_1, m_2}(\mu_a - \hat{\mu}_a)\hat{p}_1\hat{p}_2 \\
    &= SO + \underbrace{\left(\frac{\pi_a - \hat{\pi}_a}{\hat{\pi}_a}\right)\sum_{m_1, m_2}\hat{p}_1\hat{p}_2(\mu_a - \hat{\mu}_a)}_{(ii)} + \sum_{m_1, m_2}(\color{blue}\mu_a\color{black} - \color{red}\hat{\mu}_a)\hat{p}_1\hat{p}_2\color{black}
\end{align*}

Notice that when considering equations (\ref{eqn:d1}) - (\ref{eqn:d4}) the final term in red will cancel out with the corresponding term in red in \eqref{eqn:d4}. However, the term in blue now carries over. We can further decompose equations (\ref{eqn:d2})-(\ref{eqn:d4}) adding this additional remainder from above as:

\begin{align}
    \label{eqn:d5}&+ \underbrace{\left(\frac{\pi_a - \hat{\pi}_a}{\hat{\pi}_a}\right)\sum_{m_1, m_2}\hat{\mu}_a\hat{p}_2(p_1 - \hat{p}_1)}_{(iii)} + \underbrace{\left(\frac{\pi_a - \hat{\pi}_a}{\hat{\pi}_a}\right)\sum_{m_1, m_2}\hat{\mu}_a\hat{p}_1(p_2 - \hat{p}_2)}_{(iv)} \\
    \label{eqn:d6}&+ \color{blue}\sum_{m_1, m_2}\mu_a\hat{p}_1\hat{p}_2 \color{black} - \sum_{m_1, m_2}\mu_ap_1p_2 + \sum_{m_1, m_2}\hat{\mu}_a\hat{p}_2(p_1 - \hat{p}_1) + \sum_{m_1, m_2}\hat{\mu}_a\hat{p}_1(p_2 - \hat{p}_2) 
\end{align}
%
where \eqref{eqn:d6} includes the remainder from before (in blue), the $-\psi_{M_1, a}$ term, and additional remainder terms from \eqref{eqn:d5} via added and subtracted the same quantity to obtain second-order terms. We conclude by decomposing \eqref{eqn:d6}:

\begin{align*}
    &= \sum_{m_1, m_2}\color{red}\mu_a(\hat{p}_1\hat{p}_2\color{black} - p_1p_2) - \underbrace{\sum_{m_1, m_2}(\mu_a - \hat{\mu}_a)\hat{p}_2(p_1 - \hat{p}_1)}_{(v)} + \sum_{m_1, m_2} \color{red}\mu_a\hat{p}_2\color{blue}(p_1\color{black} - \color{red}\hat{p}_1\color{black}) \\
    &+ \sum_{m_1, m_2} \hat{\mu}_a\hat{p}_1(p_2 - \hat{p}_2) \\
    &= SO - \sum_{m_1, m_2} \color{red}\mu_a\color{blue} p_1\color{black} (p_2  - \color{red}\hat{p}_2\color{black}) + \sum_{m_1, m_2} \hat{\mu}_a\hat{p}_1(p_2 - \hat{p}_2) \\
    &= SO - \sum_{m_1, m_2} \mu_a p_1 (p_2  - \hat{p}_2) - \underbrace{\sum_{m_1, m_2} \hat{\mu}_a(p_1 - \hat{p}_1)(p_2 - \hat{p}_2)}_{vi} + \sum_{m_1, m_2} \hat{\mu}_a p_1(p_2 - \hat{p}_2) \\
    &= SO - \underbrace{\sum_{m_1, m_2} (\mu_a - \hat{\mu}_a)p_1(p_2 - \hat{p}_2)}_{(vii)}
\end{align*}

Thus we have shown that $P[\hat{\psi}_{M_1, a} - \psi_{M_1, a}]$ can be expressed by the sums of terms (i)-(vii), which are second-order in the nuisance estimation.

The derivation for $P[\hat{\psi}_{M_1, a'} - \psi_{M_1, a'}]$ is virtually identical. By symmetry of the problem, the result above is identical, except we replace $p_1$ with $p_1' = p(m_1 \mid a', x)$, and set term (ii) as product of errors between $(\hat{\pi}_{a'} - \pi_{a'})$ and ($\hat{p}_1' - p_1'$). 

Putting everything together, we get the following result:

\begin{align}
    \nonumber & P[\hat{\psi}_{M_1} - \psi_{M_1}] \\
    \label{eqn:m1decomp.1}&= \mathbb{E}\left[\frac{\pi_a(X)}{\hat{\pi}_a(X)}\sum_{m_1, m_2}\frac{(\hat{p}(m_1 \mid a, X) - \hat{p}(m_1 \mid a', X))\hat{p}(m_2 \mid a', X)}{\hat{p}(m_1, m_2 \mid a', X)}\right.\\
    \nonumber&\left.\times \left(p(m_1, m_2 \mid a, X) - \hat{p}(m_1, m_2 \mid a, X))(\mu_a(m_1, m_2, X) - \hat{\mu}_a(m_1, m_2, X)) \right)\right] \\
    \label{eqn:m1decomp.2}&+ \mathbb{E}\left[\left(\frac{\pi_a(X) - \hat{\pi}_a(X)}{\hat{\pi}_a(X)}\right)\sum_{m_1, m_2}\hat{p}(m_2 \mid a', X)[\hat{p}(m_1 \mid a, X) - \hat{p}(m_1 \mid a', X)] \right.\\
    \nonumber&\left.\times(\mu_a(m_1, m_2, X) - \hat{\mu}_a(m_1, m_2, X))\right] \\
    \label{eqn:m1decomp.3}&+ \mathbb{E}\left[\left(\frac{\hat{\pi}_a(X) - \pi_a(X)}{\hat{\pi}_a(X)}\right)\sum_{m_1, m_2}\hat{\mu}_a(m_1, m_2, X)\hat{p}(m_2 \mid a', X)[p(m_1 \mid a, X) - \hat{p}(m_1 \mid a, X) \right.\\
    \nonumber&\left.+ (p(m_1 \mid a', X) - \hat{p}(m_1 \mid a', X))\right] \\
    \label{eqn:m1decomp.4}&+ \mathbb{E}\left[\left(\frac{\hat{\pi}_a(X) - \pi_a(X)}{\hat{\pi}_a(X)}\right)\sum_{m_1, m_2}\hat{\mu}_a(m_1, m_2, X)\right.\\
    \nonumber&\left.\times[\hat{p}(m_1 \mid a, X) - \hat{p}(m_1 \mid a', X)][p(m_2 \mid a, X) - \hat{p}(m_2 \mid a', X)\right]\\
    \label{eqn:m1decomp.5}&- \mathbb{E}\left[\sum_{m_1,m_2}\hat{p}(m_2 \mid a', X)(\mu_a(m_1, m_2, X) - \hat{\mu}_a(m_1, m_2, X))\right.\\
    \nonumber&\left.\times(p(m_1 \mid a, X) - \hat{p}(m_1 \mid a, X) - (p(m_1 \mid a', X) - \hat{p}(m_1 \mid a', X))\right] \\
    \label{eqn:m1decomp.6}&- \mathbb{E}\left[\sum_{m_1, m_2}\hat{\mu}_a(m_1, m_2, X)[p(m_2 \mid a', X) - \hat{p}(m_2 \mid a', X)] \right. \\
    \nonumber&\left.\times (p(m_1 \mid a, X) - \hat{p}(m_1 \mid a, X) - (p(m_1 \mid a', X) - \hat{p}(m_1 \mid a', X))\right] \\
    \label{eqn:m1decomp.7}&- \mathbb{E}\left[\sum_{m_1, m_2}(p(m_1 \mid a, X) - p(m_1 \mid a', X))\right. \\
    \nonumber&\left.\times(\mu_a(m_1, m_2, X) - \hat{\mu}_a(m_1, m_2, X))(p(m_2 \mid a', X) - \hat{p}(m_2 \mid a', X) \right]
\end{align}

\section{Comparison of results}

Overall the result we derive gives an expression that is quite similar to the ones in equations (\ref{eqn:m1decomp.1})-(\ref{eqn:m1decomp.8}). For the relevant terms in $P(\hat{\psi}_a - \psi_a)$, there is one substantive difference: \eqref{eqn:m1decomp.1} is divided by $p(m_1, m_2 \mid a, X)$, whereas I do not see a reason this term should exist. Additionally, the derivation in Benkeser and Ran (2021) does not fully simplify all expressions. For example, \eqref{eqn:m1decomp.7} leaves the expression in terms of the product of errors in the outcome model and the multiplication of the marginal mediator probabilities. Perhaps this is because they are considering a continuous mediator? Regardless, we can expand out this term by adding and subtracting, for example, $\hat{p}_1p_2$ to show this in terms only of the product of errors in two nuisance functions.

On the other hand our derivation of $P(\hat{\psi}_{a'} - \psi_{a'})$ is quite a bit different: we are missing several terms. In particular, letting $p_1' = p(m_1 \mid a', X)$, the expression in (\ref{eqn:m1decomp.7})-(\ref{eqn:m1decomp.8}) does not include the following terms that we do include:

\begin{align}
    \label{eqn:missing1}&\mathbb{E}\left[\sum_{m_1, m_2}[\hat{\mu}_a - \mu_a][\hat{p}_1'\hat{p}_2 - p_1'p_2]\right] \\
    &\mathbb{E}\left[\sum_{m_1, m_2}\hat{\mu}_a[\hat{p}_1' - p_1'][\hat{p}_2 - p_2]\right]
\end{align}
%
where again we can further simply \eqref{eqn:missing1}. Notice that these equations are simply analogues (\ref{eqn:m1decomp.7})-(\ref{eqn:m1decomp.8}) for $\psi_{M_1, a'}$.

Lastly, the term in \eqref{eqn:m1decomp.1} for the $\psi_{M_1, a'}$ term is also inexplicably (I think) divided by $p(m_1, m_2 \mid a, X)$.

